On Maxwell fluid with relaxation time and viscosity depending on the pressure

We study a variant of the well known Maxwell model for viscoelastic fluids, namely we consider the Maxwell fluid with viscosity and relaxation time depending on the pressure. Such a model is relevant for example in modelling behaviour of some polymers and geomaterials. Although it is experimentally known that the material moduli of some viscoelastic fluids can depend on the pressure, most of the studies concerning the motion of viscoelastic fluids do not take such effects into account despite their possible practical significance in technological applications. Using a generalized Maxwell model with pressure dependent material moduli we solve a simple boundary value problem and we demonstrate interesting non-classical features exhibited by the model.

==> maxwell-macros.tex <==
\renewcommand{\norm}[1]{\ensuremath{\left|#1\right|}}
%\newcommand{\vhatx}{\ensuremath{v^{\hat{x}}}}
\newcommand{\tildevhatx}{\ensuremath{{\tilde{v}}^{\hat{x}}}}
\newcommand{\hatvhatx}{\ensuremath{{\hat{v}}^{\hat{x}}}}
\newcommand{\haty}{\ensuremath{\hat{y}}}

\newcommand{\sxx}{\ensuremath{\tensor{S}{_{\hat{x}\hat{x}}}}}
\newcommand{\sxy}{\ensuremath{\tensor{S}{_{\hat{x}\hat{y}}}}}
\newcommand{\syy}{\ensuremath{\tensor{S}{_{\hat{y}\hat{y}}}}}
\newcommand{\tildesxy}{\ensuremath{\tensor{\tilde{S}}{_{\hat{x}\hat{y}}}}}


\newcommand{\dsxx}{\ensuremath{\tensor*{S}{^\star_{\hat{x}\hat{x}}}}}
\newcommand{\dsxy}{\ensuremath{\tensor*{S}{^\star_{\hat{x}\hat{y}}}}}
\newcommand{\dimpi}{\ensuremath{\pi^\star}}
\newcommand{\dimbeta}{\ensuremath{\beta^\star}}
\newcommand{\dimgamma}{\ensuremath{\gamma^\star}}

\newcommand{\dvhatx}{\ensuremath{{v^{\hat{x}}}^\star}}
\newcommand{\dy}{\ensuremath{y^\star}}
\newcommand{\dt}{\ensuremath{t^\star}}
\newcommand{\dimlambda}{\ensuremath{\lambda^\star}}
\newcommand{\dimmu}{\ensuremath{\mu^\star}}

%Added by Satish
%\newcommand{\tildevhatxIm}{\ensuremath{\Im(\tildevhatx)}}
%\newcommand{\tildevhatxRe}{\ensuremath{\Re(\tildevhatx)}}
\newcommand{\tildevhatxIm}{\ensuremath{\tildevhatx_{\imagpart}}}
\newcommand{\tildevhatxRe}{\ensuremath{\tildevhatx_{\realpart}}}
\newcommand{\pfx}[2]{\pd{#1}{#2}}
\newcommand{\tfx}[2]{\dd{#1}{#2}}
\newcommand{\We}{\mathrm{We}}
\newcommand{\realpart}{\mathrm{Re}}
\newcommand{\imagpart}{\mathrm{Im}}


==> vit-prusa-macros-experimental.tex <==
\makeatletter
% \@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
% {
% \renewcommand{\tnsr@Aux}[3][]{%
% \mathpalette{\tnsr@Plt{#1}{#3}}{\mathrm #2}%
% \tnsr@Wrn
% }%\tnsr@Aux
% }{%
% \relax%
% }
% \makeatother


% operators
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\rot}{rot}
\DeclareMathOperator{\Asym}{Asym}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\signum}{sign}


% hyperbolic functions
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arccoth}{arccoth}

% big o
\newcommand{\bigo}[1]{\ensuremath{{\mathcal O}\left(#1 \right)}}

% exponential
\newcommand{\exponential}[1]{\ensuremath{{\mathrm e}^{#1}}}

% imaginary unit
\newcommand{\iunit}{\ensuremath{\mathrm{i}}}


% real and imaginary part
\newcommand{\realp}{\mathrm{real}}
\newcommand{\imagp}{\mathrm{imag}}

%\newcommand{\Real}{\Re}
%\newcommand{\Imag}{\Im}
\providecommand{\Real}{\Re}
\providecommand{\Imag}{\Im}


% predicates
\newcommand{\reference}{\mathrm{ref}}
\newcommand{\crit}{\mathrm{crit}}
\newcommand{\bydefinition}{\mathrm{def}}

% derivatives
\newcommand{\diff}{\mathrm{d}}

% body
\newcommand{\body}{{\mathcal B}}

% vectors and tensors
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\greekvec}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\tensorq}[1]{\ensuremath{\mathbb{#1}}}

\newcommand{\transpose}[1]{#1^\top}
\newcommand{\transposei}[1]{#1^{-\top}}
\newcommand{\inverse}[1]{#1^{-1}}

% Identity matrix
\newcommand{\identity}{\ensuremath{\tensorq{I}}}

% Cauchy stress
\newcommand{\cstress}{\tensorq{T}}
\newcommand{\cstressc}{\ensuremath{\mathrm T}}

\newcommand{\ecstress}{\tensorq{S}}
\newcommand{\ecstressc}{\ensuremath{\mathrm S}}

% deformation, deformation gradient
\newcommand{\deformation}{\greekvec{\chi}}
\newcommand{\fgrad}{\tensorq{F}}
\newcommand{\fgradrel}[3][]{\fgrad^{#1}_{#2}\left(#3\right)}


\newcommand{\rcg}{\tensorq{C}}
\newcommand{\rcgrel}[3][]{\rcg^{#1}_{#2}\left(#3\right)}

\newcommand{\lcg}{\tensorq{B}}
\newcommand{\lcgrel}[3][]{\lcg^{#1}_{#2}\left(#3\right)}

\newcommand{\rotation}{\tensorq{R}}
\newcommand{\rotationrel}[3][]{\rotation^{#1}_{#2}\left(#3\right)}

\newcommand{\stretchu}{\tensorq{U}}
\newcommand{\stretchurel}[3][]{\stretchu^{#1}_{#2}\left(#3\right)}

% Rivlin-Ericksen tensor
\newcommand{\rivlin}{{\tensorq{A}}}

% deviatoric part of Caychy stress
\newcommand{\dcstress}{\cstress - \left( \frac{1}{3}\Tr \cstress \right) \identity}
\newcommand{\dcstresssymb}{\cstress_{\delta}}

% mean normal stress
\newcommand{\cstressnorm}{\frac{1}{3}\Tr \cstress}

% velocity and velocity gradient, (skew)symmetric part of velocity gradient
\newcommand{\vecv}{\ensuremath{\vec{v}}}
\newcommand{\gradv}{\ensuremath{\nabla \vecv}}
\newcommand{\gradasym}{\ensuremath{ \tensorq{W}}}
\newcommand{\gradsym}{\ensuremath{ \tensorq{D}}}
\newcommand{\gradvl}{\ensuremath{ \tensorq{L}}}

\newcommand{\vecvc}{\mathrm{v}}

% velocity and velocity gradient, (skew)symmetric part of velocity gradient, COMPONENTS
\newcommand{\gradsymc}{\ensuremath{\mathrm D}}

% functionals
\newcommand{\functional}[1]{{\mathfrak #1}}
\newcommand{\history}[3]{{\functional{#1}_{#2}^{#3}}}

% base vectors
\newcommand{\bvecx}{\vec{e}_{\hat{x}}}
\newcommand{\bvecy}{\vec{e}_{\hat{y}}}
%\newcommand{\bvecz}{\vec{e}_{\hat{z}}}

\newcommand{\bvecr}{\vec{e}_{\hat{r}}}
\newcommand{\bvect}{\vec{e}_{\hat{\theta}}}
\newcommand{\bvecp}{\vec{e}_{\hat{\varphi}}}
\newcommand{\bvecz}{\vec{e}_{\hat{z}}}

% components
\newcommand{\vhatx}[1][v]{{#1}^{\hat{x}}}
\newcommand{\vhaty}[1][v]{{#1}^{\hat{y}}}
%\newcommand{\bvhatz}{\vhat{e}_{\hat{z}}}

\newcommand{\vhatr}[1][v]{{#1}^{\hat{r}}}
\newcommand{\vhatt}[1][v]{{#1}^{\hat{\theta}}}
\newcommand{\vhatp}[1][v]{{#1}^{\hat{\varphi}}}
\newcommand{\vhatz}[1][v]{{#1}^{\hat{z}}}

% base vectors, abstract covariant and contravariant basis
\newcommand{\cobvec}[1]{\vec{g}_{#1}} % covariant base vector
\newcommand{\conbvec}[1]{\vec{g}^{#1}} % contravariant base vector
\newcommand{\cobvecn}[1]{\vec{g}_{\hat{#1}}} % covariant base vector
\newcommand{\conbvecn}[1]{\vec{g}^{\hat{#1}}} % contravariant base vector

\newcommand{\mtensor}{\tensorq{g}}
\newcommand{\mtensorc}{{\mathrm g}}

% hypergeometric function
\newcommand{\hypergeom}[4]{\ensuremath{ \mathrm{F}\left( \left[#1, #2 \right]; \left[ #3 \right]; #4\right)}}

% sets
\newcommand{\R}{\ensuremath{{\mathbb R}}}
\makeatletter
\@ifpackageloaded{hyperref}% \C is defined in hyperref package
{\renewcommand{\C}{\ensuremath{{\mathbb C}}}%
}{%
\newcommand{\C}{\ensuremath{{\mathbb C}}}%
}
\makeatother
\newcommand{\Q}{\ensuremath{{\mathbb Q}}}
\newcommand{\N}{\ensuremath{{\mathbb N}}}
\newcommand{\Z}{\ensuremath{{\mathbb Z}}}

% Reynolds, Womersley number, etc.
\newcommand{\Reynolds}{\mathrm{Re}}
\newcommand{\Womersley}{\mathrm{Wo}}
\newcommand{\Rayleigh}{\mathrm{Ra}}
\newcommand{\RayleighSqrt}{\mathrm{R}}
\newcommand{\Prandtl}{\mathrm{Pr}}
\newcommand{\Grashof}{\mathrm{Gr}}
\newcommand{\Mach}{\mathrm{Ma}}
\newcommand{\Froude}{\mathrm{Fr}}
\newcommand{\Peclet}{\mathrm{Pe}}
\newcommand{\Eckert}{\mathrm{Ec}}
\newcommand{\Brinkman}{\mathrm{Br}}


% Symetric and antisymetric tensors
\newcommand{\asym}[1]{\ensuremath{\Asym \left( #1 \right)}}
\newcommand{\sym}[1]{\ensuremath{\Sym \left( #1 \right)}}

% Energy, free energy, entropy, temperature
\newcommand{\ienergy}{\ensuremath{e}}
\newcommand{\fenergy}{\ensuremath{\psi}} % free energy
\newcommand{\entropy}{\ensuremath{\eta}} % entropy
\newcommand{\temp}{\ensuremath{\theta}} % temperature
\newcommand{\temptoref}{\ensuremath{\vartheta}} % (temperature - reference temperature)/(reference temperature)


% Derivatives, partial derivatives, covariant derivatives 
\newcommand{\pd}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\ppd}[2]{\ensuremath{\frac{\partial^2 {#1}}{\partial {#2^2}}}}
\newcommand{\dd}[2]{\ensuremath{\frac{\diff {#1}}{\diff {#2}}}}
\newcommand{\cd}[2]{\ensuremath{\frac{\diff^* {#1}}{\diff {#2}}}}
\newcommand{\ddd}[2]{\ensuremath{\frac{\diff^2 {#1}}{\diff {#2}^2}}}


\newcommand{\fid}[1]{\ensuremath{\accentset{\triangledown}{#1}}}
\newcommand{\fidd}[1]{\ensuremath{\accentset{\triangledown \! \triangledown}{#1}}}

\makeatletter
\@ifpackageloaded{tensor}% tensor is a package for a better typesetting of tensors
{
\newcommand{\codev}[2]{\ensuremath{{#1}|\indices{_{#2}}}}
}{%
\newcommand{\codev}[2]{\ensuremath{\left. {#1} \right|_{#2}}}
}
\makeatother


% Bessel and Kelvin functions

\newcommand{\BesselI}[2]{\ensuremath{{\mathrm I}_{#1}\left(#2\right)}} 
\newcommand{\BesselK}[2]{\ensuremath{{\mathrm K}_{#1}\left(#2\right)}}
\newcommand{\BesselJ}[2]{\ensuremath{{\mathrm J}_{#1}\left(#2\right)}}
\newcommand{\BesselY}[2]{\ensuremath{{\mathrm Y}_{#1}\left(#2\right)}}

\newcommand\BesselRoot[2]{\ensuremath{{\rm j}_{#1,#2}}}

\newcommand{\KelvinBer}[2]{\ensuremath{{\mathrm{ber}}_{#1}\left(#2\right)}} 
\newcommand{\KelvinBei}[2]{\ensuremath{{\mathrm{bei}}_{#1}\left(#2\right)}}
\newcommand{\KelvinKer}[2]{\ensuremath{{\mathrm{ker}}_{#1}\left(#2\right)}}
\newcommand{\KelvinKei}[2]{\ensuremath{{\mathrm{kei}}_{#1}\left(#2\right)}}

% norms
\newcommand{\norm}[2][]{\ensuremath{\left\|#2\right\|_{#1}}}

% volume
\newcommand{\volume}[1][\Omega]{\ensuremath{#1}}
\newcommand{\svolume}[1][\partial\Omega]{\ensuremath{#1}}


% volume and surface integral
\newcommand{\intvolume}[2][\volume]{\int_{#1} #2\; \diff \vec{x}}
\newcommand{\intsvolume}[2][\svolume]{\int_{#1} #2\; \diff S }


% products
\newcommand{\tensortensor}[2]{\ensuremath{#1 \otimes #2}}
\newcommand{\tensordot}[2]{\ensuremath{#1 : #2}}
\newcommand{\vectordot}[2]{\ensuremath{#1 \bullet #2}}
\newcommand{\vectorcross}[2]{\ensuremath{#1 \times #2}}

% function spaces
\newcommand{\sdist}[1][\Omega]{\ensuremath{{\mathcal D}} \left(#1 \right)}
\newcommand{\sdistd}[1][\Omega]{\ensuremath{{\mathcal D}^\prime} \left(#1 \right)}

\newcommand{\scdiv}[1][\Omega]{\ensuremath{{\mathcal V}} \left(#1 \right)}

\newcommand{\loc}{\mathrm{loc}}

\newcommand{\slebl}[2]{\ensuremath{L}^{#1}_{\loc} \left(#2 \right)}
\newcommand{\sleb}[2]{\ensuremath{L}^{#1} \left(#2 \right)}


\newcommand{\ssob}[3]{\ensuremath{W}^{#1, #2} \left(#3 \right)}

% dualities, scalar products
\newcommand{\fadual}[4]{\left\langle #1, #2\right\rangle_{#3, #4}}
\newcommand{\fascal}[4]{\left\langle #1, #2\right\rangle_{#3, #4}}
